Optimal design of experiments for a lithium-ion cell: parameters identification of an isothermal single particle model with electrolyte dynamics

Advanced battery management systems rely on mathematical models to guarantee optimal functioning of Lithium-ion batteries. The Pseudo-Two Dimensional (P2D) model is a very detailed electrochemical model suitable for simulations. On the other side, its complexity prevents its usage in control and state estimation. Therefore, it is more appropriate the use of simplified electrochemical models such as the Single Particle Model with electrolyte dynamics (SPMe), which exhibits good adherence to real data when suitably calibrated. This work focuses on a Fisher-based optimal experimental design for identifying the SPMe parameters. The proposed approach relies on a nonlinear optimization to minimize the covariance parameters matrix. At first, the parameters are estimated by considering the SPMe as the real plant. Subsequently, a more realistic scenario is considered where the P2D model is used to reproduce a real battery behavior. Results show the effectiveness of the optimal experimental design when compared to standard strategies.

==> sections/introduction.tex <==
The need for energy storage devices of low weight and high energy density has been significantly increasing over the years, along with the growing demand of portable devices, battery electric vehicles and grid-connected batteries. Lithium-ion batteries exhibit the  best features in terms of high energy and power density,
high energy and coulombic efficiency, low self-discharge and negligible memory effect. Nevertheless their safe and profitable operations require suitable Advanced Battery Management Systems (ABMSs) \cite{chaturvedi2010algorithms}. These latter rely on mathematical models to guarantee high performances. Although the Electrochemical Models (EMs), such as the well known theory based Pseudo Two Dimensional (P2D) model \cite{doyledesign}, are very accurate,  their use within the context of ABMSs is challenging due  to their  computational complexity.  Besides, while their advantages for simulation purposes are apparent, their use within a control framework may be difficult, due to  observability and parameter identification issues. In this work, we address the problem of parameter identification. 
The importance of  parameters identification in battery field is also stressed by  the fact that even when the same  cell is considered, the inter-variability of the parameters can be very high, as demonstrated in \cite{ecker2015parameterization}. 
Identifiability and parameters identification have been considered within the context of batteries by several authors. In \cite{lu2013review}   an overview of different battery models and parameter identification techniques is presented, while in \cite{he2011evaluation} the parameter identification process for an Equivalent Circuit Model (ECM) is described. In \cite{torchio2015real},  a step response model, suitable for control purposes, is identified using the least squares  method, while the same authors in \cite{torchio2017design} propose a piece-wise affine approximations  of the P2D model.  The authors in \cite{bizeray2017identifiability} discuss the identifiability of the Single Particle Model (SPM, \cite{santhanagopalan2006review})  parameters, by operating a  model linearization and grouping them in hyper-parameters that can be experimentally identified. 
In \cite{lópez2016computational} a structural identifiability and a deep analysis of ill-conditioning sources  of the Doyle-Fuller-Newman (DFN, \cite{doyle1993modeling})  model is considered, based on the Fisher Information Matrix (FIM, \cite{akaike1998information}). The latter gives a measure of how informative a certain input signal is in terms of parameter sensitivity. In particular, the authors show that repeating a discharging experiment with several discharging currents may improve parameters identification process, reducing their variances.  However, some parameters of such model still result  unidentifiable if one considers only voltage   measurements during  simple experiments.  In \cite{forman2012genetic} the FIM is used to evaluate the accuracy of the DFN parameters estimated using a genetic algorithm. Also in this case some parameters result unidentifiable for that particular experimental setting. 
 %Moreover, in \cite{he2011state} an adaptive extended Kalman filter is proposed in order to simultaneously estimate states and parameters of a Thevenin ECM. 
%Parameter identification is an important topic.
For this reason, it is extremely important to design suitable experiments, so to reduce uncertainty on the parameters of the considered cell.  The Design of Experiment (DoE) in the context of batteries has been considered by
\cite{mendoza2016optimization}, in which the thermal cycle of a cell is optimized in order to estimate the entropy coefficient while reducing experimental time and maximizing the FIM. In \cite{mendoza2017maximizing} a Fisher optimization framework is considered in order to identify the parameters of an ECM coupled with a thermal model, while the authors in \cite{hametner2013state} propose an optimal design of experiment for a fuzzy model of a Li-ion cell. The importance of the accuracy of the parameters estimation for control purposes is underlined in \cite{liu2016can}.

The objective of this work is to provide an optimal strategy for designing experiments, that lead to accurate estimation of model parameters, both in terms of mean and low variance, in the shortest time possible. Taking into account the observability issues, we focus on the identification of the parameters of the SPM with electrolyte dynamics (SPMe), which is an electrochemical model suitable for control purposes \cite{moura2017battery}, while previous works on this field only investigate the optimal DoE based on ECMs. 
We rely on the fact that  the generalized inverse of the FIM provides an approximation of the covariance parameter matrix. Therefore, we aim to solve a nonlinear optimization problem in order to minimize the trace of the parameter covariance matrix, over multiple experiments, as proposed in \cite{korkel2005numerical}. The simulations highlight that the use of design of experiments, rather than standard constant current profiles, provides high benefits in terms of variance reduction and convergence to the true  values of the parameters in minimum time, when the output model is affected by zero mean gaussian error. 

However, in real life experiment the assumption of zero mean gaussian  error on the output is not always verified. For this reason, in Sec. \ref{sec:p2d_esperiment} we used the optimal  DoE procedure in order to identify the SPMe parameters   with the most accurate prediction of   the P2D model output voltage. The results show that a significant error reduction in the voltage prediction can be achieved. 

Summarizing, in this work we propose,  for the first time to the knowledge of the authors, an optimal DoE based on an electrochemical model, that seems to be a good compromise between accuracy in the voltage prediction, required for control and state estimation purposes, and parameter identifiability. We present a fair comparison of the optimal DoE approach with standard strategies, in terms of convergence of the estimated parameters to the true values and variance reduction. Furthermore, we show the benefits in terms of voltage prediction accuracy, given by the optimal DoE implied in the estimation of the parameters of a simplified model (i.e. SPMe) from the data  collected by simulating  the full order model (i.e. P2D). 

The paper is organized as follows. In Sec. \ref{sec:p2d_model} the P2D model is described in detailed, while the main equations of the SPMe are recalled in Sec. \ref{sec:spm}. In Sec. \ref{sec:method} the optimization method based on the  Fisher information is presented and in Sec. \ref{sec:case_study} the benefits of the proposed method are highlighted in simulation, when the SPMe is affected by gaussian zero mean noise. In Sec.\ref{sec:p2d_esperiment} and Sec. \ref{sec:conclusions} resume the obtained results.

==> sections/spm.tex <==
The Single Particle Model (SPM), first applied to Lithium-ion batteries field in \cite{santhanagopalan2006review}, has a wide use in battery state estimation (\cite{moura2012pde}, \cite{tanim2015state}, \cite{moura2017battery}) and control \cite{chaturvedi2010modeling}. The model consists in a reduction of the well-known Doyle-Fuller-Newman \cite{doyle1993modeling} model where the solid phase of each electrode is approximated by a single spherical particle, with an area equivalent to the one of the  solid phase in the porous electrode. In the SPM basic formulation,  the diffusion of the electrolyte concentration  and the thermal effects are ignored.  In the following, the main model equations are presented and the index $i \in \{p,n\}$ is used to refer to the cathode or to the anode. The diffusion of the ion concentration $c_i(t,r_i)$  within the electrodes is described by the Fick's law
\begin{align}\label{eq:PDE}
\frac{\partial c_i(t,r_i)}{\partial t}=\frac{D_i}{r^2_i} \frac{\partial}{\partial r_i} \left( r^2_i \frac{\partial c_i(t,r_i)}{\partial r_i} \right)
\end{align}
where $t \in \mathbb{R}^+$ is the time, $r_i$ is the radial coordinate, $D_i$ is the diffusion coefficient assumed uniform within the electrode. The input current $I_{app}(t)$ enters the model in the boundary conditions
\begin{align*} 
\left. \frac{\partial c_i(t,r_i)}{\partial r_i}\right|_{r_i=0}=0 \hspace{1cm} D_i\left.\frac{\partial c_i(t,r_i)}{\partial r_i}\right|_{r_i=R_i}=-j_i
\end{align*}
where $j_p=-\frac{I_{app}(t)}{a_p\delta_p F A}$ and $j_n=\frac{I_{app}(t)}{a_n\delta_n F A}$, $F$ is the Faraday's constant, $A$ is the electrode  surface area, $a_i=\frac{3 \epsilon_i}{R_i}$ is the specific active surface area, $\epsilon_i$ is the volume fraction of the active material, $R_i$ is the particle radius, $\delta_i$ is the electrode thickness and the initial condition equation is
\begin{align*}
c_i(0,r_i)=c^0_i(r_i)
\end{align*} 
where $c^0_i(r_i)$ is the initial concentration profile over the radial axis. 
Although the SPM is less accurate  than other electrochemical models, especially in presence of high current density and low electrolyte conductivity, due to its simplicity it is particularly suitable for battery state estimation and control.
\subsection{Simplified SPM} \label{sec:SPM_simplified}
In order to further reduce the complexity of the model, it is possible to replace  the partial differential equation in \eqref{eq:PDE} with  a set of Ordinary Differential Equations (ODEs). As discussed in \cite{subramanian2005efficient},  the lithium concentration profile in the particles can be approximated as a polynomial function
\begin{align*}
c_i(t,r_i)=a(t)+b(t)\frac{r^2_i}{R^2_i}+d(t)\frac{r^4_i}{R^4_i}
\end{align*}
where $a(t)$, $b(t)$, $d(t)$ are expressed in terms of  volume-averaged lithium concentration $\overline{c}_i(t)$,  volume-averaged concentration flux $\overline{q}_i(t)$ and surface concentration $c_{s,i}(t)$. In particular, the Fick's law is reduced to a set of four ODEs 
\begin{subequations}\label{eq:diff_states}
\begin{align} 
\dot{\overline{c}}_p(t)&= \frac{3}{R_pFAs_p}I_{app}(t)\\
\dot{\overline{c}}_n(t)&= -\frac{3}{R_nFAs_n}I_{app}(t)\\
\dot{\overline{q}}_p(t)&=-30 \frac{D_p}{R^2_p}\overline{q}_p(t)+\frac{45}{2R^2_p}\frac{1}{FAs_p}I_{app}(t)\\ 
\dot{\overline{q}}_n(t)&=-30 \frac{D_n}{R^2_n}\overline{q}_n(t)-\frac{45}{2R^2_n}\frac{1}{FAs_n}I_{app}(t)
\end{align}
\end{subequations}
where $s_i=a_i\delta_i$, while the positive and negative surface concentrations are given by
\begin{align*}
c_{s,p}(t)&=\overline{c}_p(t)+\frac{8R_p}{35}\overline{q}_p(t)+\frac{R_p}{35D_p}\frac{1}{FAs_p}I_{app}(t)\\
c_{s,n}(t)&=\overline{c}_n(t)+\frac{8R_n}{35}\overline{q}_n(t) -\frac{R_n}{35D_n}\frac{1}{FAs_n}I_{app}(t)
\end{align*}
The output voltage  is a nonlinear function of  the states and the input
\begin{align*}
y(t)&=\eta_p(t)-\eta_n(t)+U_p(\theta_p(t))-U_n(\theta_n(t))
\end{align*}
where $\eta_p$ and $\eta_n$ are the positive and negative overpotentials, respectively defined as 
\begin{align*}
\eta_p(t)&=\beta \sinh^{-1} \left(  \frac{-I_{app}(t)}{2AFs_pk_p\sqrt{c^0_e \, c_{s,p}(t) \left(c^{max}_p-c_{s,p}(t)\right)}} \right)\\
\eta_n(t)&=\beta \sinh^{-1} \left(  \frac{I_{app}(t)}{2AFs_nk_n\sqrt{c^0_e \, c_{s,n}(t) \left(c^{max}_n-c_{s,n}(t)\right)}} \right)
\end{align*}
where $\beta=\frac{2RT}{F}$,   $k_p$ and $k_n$ are the positive and negative reaction rate constants, $c^{max}_p$ and $c^{max}_n$ are the positive and negative maximum solid-phase concentrations, $c^0_{e}$ is the  electrolyte concentration assumed to be constant, while $U_p$ and $U_n$ are  the positive and negative open circuit potentials
\begin{align*}
U_p(\theta_p)=&\frac{f_1+f_2  \theta_p^2 +f_3\theta_p^4 + f_4 \theta_p^6 +f_5 \theta_p^8 + f_6 \theta_p^{10}}{f_7+f_8 \theta_p^2+f_9 \theta_p^4+f_{10} \theta_p^6+f_{11} \theta_p^8+f_{12} \theta_p^{10}} \\
\begin{split}
U_n(\theta_n)=& g_1 + g_2 \theta_n + g_3 \theta_n^{0.5} + \frac{g_4}{\theta_n} + \frac{g_5}{\theta_n^{1.5}} +  \\&+ g_6e^{(g_7+g_8\theta_n)}+g_9 e^{(g_{10} \theta_n +g_{11})}
\end{split}
\end{align*} 
described by nonlinear empirical functions of positive and negative  surface stoichiometries, respectively given by
\begin{align*}
\theta_p(t)=\frac{c_{s,p}(t)}{c_p^{max}} \hspace{1cm}
\theta_n(t)=\frac{c_{s,n}(t)}{c_n^{max}}
\end{align*}
Finally the State of Charge (SOC) is defined as
\begin{align*}
SOC(t)=\frac{100}{c^{max}_p}\left( \frac{\overline{c}_p(t)- \theta_p^{min} c^{max}_p }{\theta_p^{max}-\theta_p^{min}} \right)
\end{align*}
where $\theta_p^{min}$ and $\theta_p^{max}$ are the minimum and maximum positive surface stoichiometries. 
\subsection{Model parameters and constants}
All the constants, the model parameters  and the  coefficients of  $U_p$ and $U_n$ have been taken from  real battery data  \cite{northrop2011coordinate} and   summarized in  Tab. \ref{tab:parameters_fixed}, Tab. \ref{tab:parameters_estimated}, Tab. \ref{tab:coefficienti_Up} and Tab. \ref{tab:coefficienti_Un}. The measurement units are chosen in a way such that the derivatives in \eqref{eq:diff_states} have reasonable and comparable values. 

\begin{table} [htpb] 
\begin{center}
{\renewcommand\arraystretch{1.4} 
\begin{tabular}{|c|c|c|} 
\hline
Parameter  & Value & Unit\\
\hline
$T$ & 298.15 & $K$\\
\hline
$F$ & $9.6487 \cdot 10^{-8}$ & $\frac{C}{pmol}$ \\
\hline
$R$ & $8.314 \cdot 10^{-12}$ & $\frac{J}{pmol}$ \\
\hline
$A$  & $2.05 \cdot 10^{12}$ & $\mu m^2$\\
\hline
$R_p$, $R_n$  &  2 & $\mu m$  \\
%\hline
%$R_n$ &  2 & $\mu m$  \\
\hline
$c^0_e$  & $10^{-3}$ & $\frac{pmol}{\mu m^3}$ \\
\hline
$c^{max}_p $ & $5.1554\cdot 10^{-2}$ & $\frac{pmol}{\mu m^3}$ \\
\hline
$c^{max}_n$  & $3.0555\cdot 10^{-2}$ & $\frac{pmol}{\mu m^3}$ \\
\hline
$\theta_p^{min}$ & 0.99174 & -\\
\hline
$\theta_p^{max}$ & 0.49550 & -\\
\hline

\end{tabular}}
\end{center}
\caption{Value of  constants and  parameters.}\label{tab:parameters_fixed}
\end{table}

\begin{table} [htpb] 
\begin{center}
{\renewcommand\arraystretch{1.4} 
\begin{tabular}{|c|c|c|c|} 
\hline
Parameter  & Initial guess $\phi_0$ & True value $\phi^\star$ & Unit\\
\hline
$s_p$ & 40.1672 & 36.2673 & -  \\
\hline
$s_n$ & 49.4500 & 36.1800 & - \\
\hline
$D_p$ & 0.0055 & 0.01 & $\frac{\mu m^2}{s}$\\
\hline
$D_n$ & 0.0457 & 0.0390 & $\frac{\mu m^2}{s}$ \\
\hline
$k_p$ & 0.0248 & 0.0233 & $\frac{\mu m^{2.5}}{pmol^{0.5}s} $\\
\hline
$k_n$ & 0.0372 & 0.0503 & $\frac{\mu m^{2.5}}{pmol^{0.5}s} $ \\
\hline
\end{tabular}}
\end{center}
\caption{Initial guess and true value of the parameters to be estimated.}\label{tab:parameters_estimated}
\end{table}

\begin{table} [htpb] 
\begin{center}
{\renewcommand\arraystretch{1.4} 
\begin{tabular}{|c|c|c|c|c|c|} 
\hline
$f_1$ & -4.656 & $f_5$ & - 462.471 & $f_9$ & -79.532\\
\hline
$f_2$ & 88.669 & $f_6$ & 433.434 & $f_{10}$ & 37.311  \\
\hline
$f_3$ & - 401.119 & $f_7$ & -1 & $f_{11}$ & -73.083 \\
\hline
$f_4$ & 342.909 & $f_8$  & 18.933 & $f_{12}$ & 95.96 \\
\hline
\end{tabular}}
\end{center}
\caption{Coefficients of  positive open circuit potential.}\label{tab:coefficienti_Up} 
\end{table}
\begin{table} [htpb] 
\begin{center}
{\renewcommand\arraystretch{1.4} 
\begin{tabular}{|c|c|c|c|c|c|} 
\hline
$g_1$ & 0.722 & $g_5$ & 0.0019 & $g_9$ & -0.798 \\
\hline
$g_2$ & 0.138 &$g_6$ & 0.2808 & $g_{10}$ & 0.4465 \\
\hline
$g_3$ & 0.029 & $g_7$ & 0.9 & $g_{11}$ & -0.4108 \\
\hline
$g_4$ & -0.0172 & $g_8$ & -15 & - & - \\
\hline
\end{tabular}}
\end{center}
\caption{Coefficients of  negative open circuit potential.}\label{tab:coefficienti_Un} 
\end{table}


